Advances in Trajectory Optimization for Space Vehicle Control

Space mission design places a premium on cost and operational efficiency. The search for new science and life beyond Earth calls for spacecraft that can deliver scientific payloads to geologically rich yet hazardous landing sites. At the same time, the last four decades of optimization research have put a suite of powerful optimization tools at the fingertips of the controls engineer. As we enter the new decade, optimization theory, algorithms, and software tooling have reached a critical mass to start seeing serious application in space vehicle guidance and control systems. This survey paper provides a detailed overview of recent advances, successes, and promising directions for optimization-based space vehicle control. The considered applications include planetary landing, rendezvous and proximity operations, small body landing, constrained attitude reorientation, endo-atmospheric flight including ascent and reentry, and orbit transfer and injection. The primary focus is on the last ten years of progress, which have seen a veritable rise in the number of applications using three core technologies: lossless convexification, sequential convex programming, and model predictive control. The reader will come away with a well-rounded understanding of the state-of-the-art in each space vehicle control application, and will be well positioned to tackle important current open problems using convex optimization as a core technology.

==> optimization.tex <==
\makeatletter

\def\emptyCaption{{\color{white}?}}

\def\optiPadding{1mm}
\def\captionPadding{1mm}

\newcommand{\clonelabel}[2]{\@bsphack
  \expandafter\ifx\csname r@#2\endcsname\relax
  \else\protected@write\@auxout{}{\string\newlabel{#1}%
    {\csname r@#2\endcsname}}%
  \fi
  \expandafter\ifx\csname r@#2@cref\endcsname\relax
  \else\protected@write\@auxout{}{\string\newlabel{#1@cref}%
    {\csname r@#2@cref\endcsname}}%
  \fi
  \@esphack}

\newcounter{ProblemCounter}
\newcounter{EqStartCounter}
\newcounter{ll}
\newcounter{jj}
\newcounter{kk}

\setcounter{ProblemCounter}{0}
\setcounter{EqStartCounter}{0}

\newcommand{\setBound}[2][true]{%
  % #1: apply \tikzmark if true
  % #2: tikzmark label
  \ifthenelse{\equal{#1}{true}}{
    \tikzmark{#2\theProblemCounter}
  }{}
}
\newcommand{\getBound}[1]{pic cs:#1\theProblemCounter}

\newlength{\lineHeight}

\newcommand{\theBackground}[5]{%
  % #1: \border
  % #2: type {cost,constraint}
  % #3: cost OR constraint list
  % #4: constraint number (only relevant if type=constraint)
  % #5: \@caption
  \begin{tikzpicture}[remember picture,overlay]%
    % Styles
    \ifthenelse{\equal{#1}{true}}
    {\def\opacityValue{1}}
    {\def\opacityValue{0}}
    \tikzset{
      background/.append style={
        rectangle,
        anchor=south west,
        fill=yellow!20,
        inner sep=0,
        outer sep=0,
        minimum width=\problemWidth+2*\optiPadding,
        opacity=\opacityValue
      },
      outline box/.append style={
        anchor=south west,
        inner sep=0,
        outer sep=0
      },
      border/.append style={
        solid,
        draw=orange!80,
        line width=0.2mm,
        opacity=\opacityValue
      },
      border cap/.append style={
        background,
        border,
        anchor=west,
        minimum height=2*\optiPadding,
        rounded corners=\optiPadding,
        opacity=\opacityValue
      }
    }
    % Cost background
    \ifthenelse{\equal{#2}{cost}}{
      \phantomoutline{#3}
      \edef\costBelowShift{\belowShift}
      \path let
      \p1=(\getBound{cost.south west}),
      \p2=(\getBound{variables.south west})
      in \pgfextra{
        \node[
        background,
        minimum height=\totalHeight
        ] (cost) at (\x1-\optiPadding,\y1-\belowShift) {};
        \draw[border] (cost.south west) to (cost.north west);
        \draw[border] (cost.south east) to (cost.north east);
      };
      % Draw the top cap
      \begin{scope}
        \clip
        ($(cost.north west)+(-\optiPadding,0)$)
        rectangle
        ($(cost.north east)+(2*\optiPadding,2*\optiPadding)$);
        \node[border cap] at (cost.north west) {};
      \end{scope}
      \xdef\lastLine{cost}
      % Caption
      \ifthenelse{\equal{\writeCaption}{true}}{
        \node[
        anchor=south east,
        align=right,
        inner sep=0,
        outer sep=0,
        font={\bfseries\footnotesize\baselineskip=1.3em}
        ] (problemLabel) at ($(cost.south west)+
        (-\captionPadding,\costBelowShift*1pt)$)
        {\ifthenelse{\equal{\@tag}{}}{Problem \theequation.}{Problem \@tag.}};
        \node[
        anchor=north east,
        align=right,
        inner sep=0,
        outer sep=0,
        font={\itshape\footnotesize\baselineskip=1.3em}
        ] (description) at ($(problemLabel.south east)+(0,-2*\captionPadding)$)
        {#5};
      }{}
    }{}
    % Constraint background
    \ifthenelse{\equal{#2}{constraint}}{
      \coordinate (previous) at (\lastLine.south west);
      \phantomoutline{#3[#4]}
      \path let
      \p1 = (\getBound{constraint#4.south west}),
      \p2 = (previous)
      in \pgfextra{
        \tikzset{
          marker/.append style={
            inner sep=0,
            outer sep=0,
            minimum size=1mm,
            fill=black,
            circle
          }
        }
        \ifthenelse{\equal{#4}{\listlen#3[]}}{\tikzmath{\padExtraBelow=0;}}%
        {\tikzmath{\padExtraBelow=\optiPadding;}}
        \pgfmathparse{\y1<\y2 ? 1 : 0}
        \ifthenelse{\pgfmathresult>0}{
          \tikzmath{\lineHeight=\y2-(\y1-\belowShift)+\padExtraBelow;}
        }{
          \tikzmath{\lineHeight=\totalHeight+2*\padExtraBelow;}
        }
        \tikzmath{\constraintBgShiftX=\costResultWidth+\optiPadding;}
        \node[
        background,
        minimum height=\lineHeight
        ] (constraint#4) at (\x1-\constraintBgShiftX,\y1-\belowShift-\padExtraBelow) {};
        \draw[border] (constraint#4.south west) to (constraint#4.north west);
        \draw[border] (constraint#4.south east) to (constraint#4.north east);
      };
      \xdef\lastLine{constraint#4}
      % Draw the bottom cap
      \ifthenelse{\equal{#4}{\listlen#3[]}}{
        \begin{scope}
          \clip
          ($(\lastLine.south west)+(-\optiPadding,0)$)
          rectangle
          ($(\lastLine.south east)+(2*\optiPadding,-2*\optiPadding)$);
          \node[border cap] at (\lastLine.south west) {};
        \end{scope}
      }{}
    }{}
  \end{tikzpicture}%
}

\newcommand{\printCost}[6][true]{
  % #1: print with \setBound and alignment if true
  % #2: \result
  % #3: \constrained
  % #4: \task
  % #5: \variables
  % #6: \objective
  \setBound[#1]{cost.south west}%
  \ifthenelse{\equal{#2}{}}{}{#2=}%
  \setBound[#1]{cost.south west2}%
  \ifthenelse{\equal{#3}{true}}{\ifthenelse{\equal{#1}{true}}{&}{}}{}%
  #4_{\setBound[#1]{variables.south west}#5\setBound[#1]{bottom}}#6%
  \setBound[#1]{cost.south east}%
  \ifthenelse{\equal{#3}{true}}{%
    ~\mathrm{s.t.}\setBound[#1]{cost.south east}
  }{}%
  % determine width of the "result =" part
  \begin{tikzpicture}[remember picture,overlay]%
    \path let
    \p1=(\getBound{cost.south west}),
    \p2=(\getBound{cost.south west2})
    in \pgfextra{
      \tikzmath{\costResultWidth=\x2-\x1;}
      \xdef\costResultWidth{\costResultWidth}
    };
  \end{tikzpicture}%
}

\newcommand{\OPTBG}[4]{%
  \theBackground%
  {\border}%
  {#1}%
  {#2}%
  {#3}%
  {#4}
}

\newcommand{\theProblem}[8]{
  % #1: \result
  % #2: \constrained
  % #3: \task
  % #4: \variables
  % #5: \objective
  % #6: list of constraints
  % #7: \@label
  % #8: \@caption
  % Print the optimization problem
  \OPTBG{cost}{\printCost[false]{#1}{#2}{#3}{#4}{#5}}{0}{#8}%
  \printCost[true]{#1}{#2}{#3}{#4}{#5}%
  \ifthenelse{\equal{#7}{}}{}{\label{eq:#7_a}}
  \ifthenelse{\equal{#2}{true}}{%
    \\%
    \forloop{kk}{0}{\arabic{kk}<\listlen#6[]}{%
      \setcounter{jj}{\value{kk}+1}%
      \setcounter{ll}{\value{kk}+2}%
      &\setBound{constraint\arabic{jj}.south west}%
      \OPTBG{constraint}{#6}{\arabic{jj}}{}%
      #6[\arabic{jj}]%
      \setBound{constraint\arabic{jj}.south east}%
      \ifthenelse{\equal{#7}{}}{}{\label{eq:#7_\alph{ll}}}%
      \ifthenelse{\equal{\arabic{jj}}{\listlen#6[]}}{}{\\}
    }
  }{}
}

\newcommand{\phantomoutline}[1]{
  % \node[outline box] (outline) at (\getBound{cost.south west})
  % {\phantom{$\displaystyle#1$}};
  \node[
  draw=none,
  inner sep=0
  ] (outline) at (0,0)
  {\pgfmark{eqstart\theEqStartCounter}\phantom{$\displaystyle#1$}};
  % \node[
  % draw=black,
  % inner sep=0
  % ] (outline) at (5,0) {\pgfmark{eqstart\theEqStartCounter}{$\displaystyle#1$}};
  \path let
  \p1=(outline.north east),
  \p2=(outline.south east),
  \p3=(pic cs:eqstart\theEqStartCounter)
  in \pgfextra{
    \tikzmath{
      \totalHeight=\y1-\y2;
      \belowShift=\y3-\y2;}
    \xdef\totalHeight{\totalHeight}
    \xdef\belowShift{\belowShift}
  };
  \stepcounter{EqStartCounter}
}

\newcommand{\computeProblemWidth}[2]{
  % #1: \constrained
  % #2: list of constraints
  % Compute the problem width
  \begin{tikzpicture}[remember picture,overlay]
    \path let
    \p1=(\getBound{cost.south west}),
    \p2=(\getBound{cost.south east})
    in \pgfextra{
      \tikzmath{\problemWidth=\x2-\x1;}
      \xdef\problemWidth{\problemWidth}
    };
    \ifthenelse{\equal{#1}{true}}{
      \foreach \i in {1,...,\listlen#2[]} {
        \path let
        \p1=(\getBound{cost.south west}),
        \p2=(\getBound{constraint\i.south east})
        in \pgfextra{
          \tikzmath{\problemWidth=max(\problemWidth,\x2-\x1);}
          \xdef\problemWidth{\problemWidth}
        };
      }
    }{}
  \end{tikzpicture}
}

\define@key{optimusKeys}{task}{\def\task{#1}}%
\define@key{optimusKeys}{objective}{\def\objective{#1}}%
\define@key{optimusKeys}{variables}{\def\variables{#1}}%
\define@key{optimusKeys}{result}{\def\result{#1}}%
\define@key{optimusKeys}{border}{\def\border{#1}}%
\define@key{optimusKeys}{label}{\def\@label{#1}}%
\define@key{optimusKeys}{tag}{\def\@tag{#1}}%
\define@key{optimusKeys}{caption}{\def\@caption{#1}}%
%
\define@key{optimusKeys}{plabel}{\def\@label{#1}}% DEPRECATED, use {label}
\define@key{optimusKeys}{ptag}{\def\@tag{#1}}% DEPRECATED, use {tag}
\define@key{optimusKeys}{pcaption}{\def\@caption{#1}}% DEPRECATED, use {caption}
%
\NewEnviron{optimus}[1][]{%
  % Parameters
  \setkeys{optimusKeys}{plabel=,#1}%
  \setkeys{optimusKeys}{label=,#1}%
  \setkeys{optimusKeys}{border=false,#1}%
  \setkeys{optimusKeys}{task=\min,#1}%
  \setkeys{optimusKeys}{objective=,#1}%
  \setkeys{optimusKeys}{variables=,#1}%
  \setkeys{optimusKeys}{result=,#1}%
  \setkeys{optimusKeys}{ptag=,#1}%
  \setkeys{optimusKeys}{tag=,#1}%
  \setkeys{optimusKeys}{pcaption=,#1}
  \setkeys{optimusKeys}{caption=,#1}
  %
  % Prepare variables
  \stepcounter{ProblemCounter}%
  \ifthenelse{\equal{\BODY}{}}{%
    \xdef\constrained{false}}{%
    \xdef\constrained{true}
    \setsepchar{\#}%
    \readlist\constraints{\BODY}}
  \ifthenelse{\equal{\@caption}{}}{
    \xdef\writeCaption{false}}{
    \xdef\writeCaption{true}}
  % Print the problem
  \computeProblemWidth{\constrained}{\constraints}%
  \newcommand{\printProblemBody}{
    \theProblem%
    {\result}%
    {\constrained}%
    {\task}%
    {\variables}%
    {\objective}%
    {\constraints}%
    {\@label}%
    {\@caption}
  }
  \ifthenelse{\equal{\constrained}{true}}{
    \ifthenelse{\equal{\@label}{}}{
      \begin{align*}
        \printProblemBody
      \end{align*}
    }{
      \ifthenelse{\equal{\@tag}{}}{
        \begin{subequations}
          \label{problem:\@label}
          \begin{align}
            \printProblemBody
          \end{align}
        \end{subequations}
      }{
        \begin{taggedsubequations}{\@tag}
          \label{problem:\@label}
          \begin{align}
            \printProblemBody
          \end{align}
        \end{taggedsubequations}
      }
    }
  }{
    \ifthenelse{\equal{\@label}{}}{
      \begin{equation*}
        \printProblemBody
      \end{equation*}
    }{
      \begin{equation}
        \printProblemBody
      \end{equation}\clonelabel{problem:\@label}{eq:\@label_a}
    }
  }
}

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

